Improving the Privacy and Practicality of Objective Perturbation for Differentially Private Linear Learners

In the arena of privacy-preserving machine learning, differentially private stochastic gradient descent (DP-SGD) has outstripped the objective perturbation mechanism in popularity and interest. Though unrivaled in versatility, DP-SGD requires a non-trivial privacy overhead (for privately tuning the model's hyperparameters) and a computational complexity which might be extravagant for simple models such as linear and logistic regression. This paper revamps the objective perturbation mechanism with tighter privacy analyses and new computational tools that boost it to perform competitively with DP-SGD on unconstrained convex generalized linear problems.

==> def.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors

\usepackage{amsmath}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{caption}

\usepackage[toc,page,header]{appendix}
\usepackage{minitoc}

\usepackage{subcaption}

\usepackage{microtype}
\usepackage{graphicx}
% \usepackage{subfigure}
\usepackage{booktabs}

\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{xfrac}

\usepackage{hyperref}

\DeclareMathOperator*{\argmin}{arg\,min}

\renewcommand \thepart{}
\renewcommand \partname{}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\newcommand{\yw}[1]{\textcolor{cyan}{[yu-xiang: #1]}}

\newcommand{\rr}[1]{\textcolor{magenta}{[rachel: #1]}}
\newcommand{\ak}[1]{\textcolor{blue}{[antti: #1]}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\norm}[1]{\Vert #1 \Vert}
\numberwithin{equation}{section}
\newcommand{\ee}{{\rm e}\hspace{1pt}}
\newcommand{\ii}{\text{i}\hspace{1pt}}
\newcommand{\dd}{\hspace{1pt}{\rm d}\hspace{0.5pt}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\eps}{\epsilon}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\E{\mathbb{E}}
\def\P{\mathbb{P}}
\def\Cov{\mathrm{Cov}}
\def\Var{\mathrm{Var}}
\def\half{\frac{1}{2}}
\def\th{\mathrm{th}}
\def\tr{\mathrm{tr}}
\def\df{\mathrm{df}}
\def\dim{\mathrm{dim}}
\def\col{\mathrm{col}}
\def\row{\mathrm{row}}
\def\nul{\mathrm{null}}
\def\rank{\mathrm{rank}}
\def\nuli{\mathrm{nullity}}
\def\sign{\mathrm{sign}}
\def\supp{\mathrm{supp}}
\def\diag{\mathrm{diag}}
\def\aff{\mathrm{aff}}
\def\hy{\hat{y}}
\def\ty{\tilde{y}}
\def\hbeta{\hat{\beta}}
\def\tbeta{\tilde{\beta}}
\def\htheta{\hat{\theta}}
\def\halpha{\hat{\alpha}}
\def\hf{\hat{f}}
\def\lone{1}
\def\ltwo{2}
\def\linf{\infty}
\def\lzero{0}
\def\T{^T}
\def\R{\mathbb{R}}
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cP{\mathcal{P}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}
\def\TV{\mathrm{TV}}

==> proofs/gradient_clipping.tex <==
\section{Gradient Clipping}

For the linear and logistic regression experiments, we construct the implicit "clipped-gradient" loss function $L_C(\theta; Z)$ described in Section~\ref{section:computational_tools}. From \citet{song2020evading}, we can define this function precisely.

Consider the transformation $f(\langle x, \theta \rangle; y) := \ell(\theta; z)$. When $f(\langle x, \theta \rangle; y) = \frac{1}{2}(y - x^T \theta)^2$ is the linear loss function,
\begin{align*}
f_C(\langle x, \theta \rangle; y)= \begin{cases} 
- \frac{B}{||x||_2}\big[ \langle x, \theta \rangle - (y -  \frac{B}{||x||_2})\big] + f\big(y - \frac{B}{||x||_2}\big), \text{ for } \langle x, \theta \rangle \in (-\infty, y - \frac{B}{||x||_2}) \\
f(\langle x, \theta \rangle), \text{ for } \langle x, \theta \rangle \in (y - \frac{B}{||x||_2}, y + \frac{B}{||x||_2}) \cap \mathbb{R} \\
 \frac{B}{||x||_2}\big[ \langle x, \theta \rangle - (y +  \frac{B}{||x||_2})\big] + f\big(y + \frac{B}{||x||_2}\big), \text{ for } \langle x, \theta \rangle \in (y + \frac{B}{||x||_2}, \infty)
\end{cases}
\end{align*}

where $f\big(y - \frac{B}{||x||_2}\big) = \frac{B^2}{2||x||_2^2}$ and $f\big(y + \frac{B}{||x||_2}\big) = \frac{1}{2}\left(-\frac{B}{||x||_2}\right)^2 = \frac{B^2}{2||x||_2^2}$.

It is the same story for linear regression, except $f(\langle x, \theta \rangle; y) = -y x^T \theta + \log(1 + e^{x^T\theta})$ is the logistic loss function and we swap in $z_1 = \sigma^{-1}\left(y - \frac{B}{||x||_2}\right)$ and $z_2 = \sigma^{-1}\left(y + \frac{B}{||x||_2}\right)$ as the boundary points.



% \begin{proof}[Proof of Theorem~\ref{thm:beta_smoothness}]
% Consider the piecewise function defined in Lemma 5.1 of \citet{song2020evading}. We can then proceed in a case-by-case basis.

% When $y \in [y_1, y_2] \cap \mathbb{R}$, $g_{*}(y) = f(y)$ and so $\nabla^2 g_{*}(y) =  \nabla^2 f(y) < \beta$. When $y \in (-\infty, y_1) \cup (y_2, \infty)$, $\nabla^2 g_{*}(y) = 0$ because $\minusplus \frac{B}{||x||_2}(y - y_1) + f(y_1)$ is linear in $y$.

% Lastly, the Jacobian is undefined at $y = y_1$ and $y = y_2$. The set $\{y_1, y_2\}$ is finite and therefore has measure 0. Moreover, for the objective perturbation mechanism $\hat{\theta}^P(Z)$ we can use the bijection $b(\theta; Z)$ between the mechanism output and the noise vector to show that $\text{Pr}[\theta = b^{-1}(\{y_1, y_2\})] = 0$.
% \end{proof}

==> sections/old_experiments.tex <==
% !TEX root = ../main.tex

In this section we evaluate Algorithm~\ref{alg:comp_objpert} against DP-SGD on both linear and logistic regression.

We implement DP-SGD using Opacus \citep{yousefpour2021opacus}, and calibrate the noise using \citet{autodp} via an RDP accountant for Poisson-sampled Gaussian mechanisms (DP-SGD). %In particular, we use the improved RDP bound for the subsampled Gaussian mechanism given in Theorem 27 of \citet{wang2019subsampled}.

\subsection{Hyperparameter tuning}

The noise calibration typically used for DP-SGD is in fact optimistic. \citet{papernot2021hyperparameter} (in a follow-up work to \citet{liu2019private}) introduce and provide bounds for a private selection algorithm that pays a constant privacy cost for testing many hyperparameter candidates, by reworking the number $K$ of candidates from a fixed value to a random variable.

Table~\ref{table:select_scale} compares the noise scale of DP-SGD to DP-SGD with private selection, demonstrating that naive DP-SGD underestimates the noise level required to preserve privacy when accounting for the privacy cost of hyperparameter tuning. 

We emphasize that our results on DP-SGD are incompatible to existing work in that we conducted honest (differentially private) hyperparameter tuning. One of the take-home messages of the paper is that when we require formal end-to-end differential privacy, many results in the empirical evaluation of DP algorithms in the literature that do not account for the cost of hyperparameter tuning might be overly optimistic, thus should be taken with a grain of salt.

\begin{table}[t]
\centering
\begin{tabular}{||c c c ||} 
 \hline
 Privacy budget $\epsilon$ &  DP-SGD & Private Selection  \\ [0.5ex] 
 \hline\hline
 10   & 0.059 & 0.6  \\ 
 \hline
 1  & 0.15 & 1.81  \\
 \hline
 0.1  & 1.08 & 14.54    \\
 \hline
\end{tabular}
 \caption{Comparison of noise scale between DP-SGD with (rightmost column) and without (middle column) private selection. The noise is calibrated with $\delta=1e-5$, clipping threshold $C = 0.1$, number of iterations $T=1000$, and sampling probability $p = 0.1$. For private selection, we use the logarithmic distribution with $\eta = 0$ and $\gamma = 0.5$.}
\end{table}
\label{table:select_scale}

% show the noise scale and explain the optimism

\subsection{Logistic Regression}
\label{section:logistic_regression}
We evaluate the performance of Algorithm~\ref{alg:comp_objpert} on the UCI Adult dataset \citep{kohavi1996scaling}. The classification task  is to predict whether a person's income exceeds \$50K a year.

We fix $\delta=1e-5$ and vary $\epsilon \in [0.1, 1, 8]$. For Algorithm~\ref{alg:comp_objpert}, we set $\sigma_{out} = 0.1 \tau = 0.005,$ and $C = 1$; the parameters of the logistic loss function are $L = 1$ and $\beta = 0.25$. Because we don't clip the gradients for Algorithm~\ref{alg:comp_objpert} in this experiment ($C = L$), we first pre-process the Adult dataset by normalizing each row $x_i := \dfrac{x_i}{||x_i||_2^2}$. We use the L-BFGS optimizer to find an approximate solution to the perturbed objective.

We run DP-SGD with 100 epochs, clipping threshold $C = 0.1$ and an expected batch size of 64. We then calculate the number of iterations $T$ as the product of the number of epochs and the number of batches, and calibrate the noise scale $\sigma$ to achieve the desired privacy guarantee. We train the model using each candidate learning rate and then report the best accuracy on the test set.

Results in Figure~\ref{fig:adult} are averaged over $30$ trials.

\begin{figure}[h]
\centering
\includegraphics[width=.93\columnwidth]{figures/adult_plot.png}
         \caption{Logistic regression on UCI Adult dataset.}
\end{figure}
\label{fig:adult}

\subsection{Linear Regression}
We next use the UCI wine quality dataset to evaluate the performance of Algorithm~\ref{alg:comp_objpert} on a regression task to predict wine quality on a scale from 1 to 10.

We run DP-SGD with the same setup as described in Section~\ref{section:logistic_regression}. For Algorithm~\ref{alg:comp_objpert}, we set $\tau = 0.005$ and $\sigma_{out} = 0.01$ for $\epsilon \in [1, 8]$; for $\epsilon = 0.1$ we need to set $\sigma_{out} = 0.02$ to satisfy DP. For the linear loss function, $\beta = 1$ and $L$ is undefined in the unconstrained setting; we set $C = 0.1$ to enforce a bound on the gradients. Using L-BFGS with clipped gradients requires us to implement the clipped-gradient loss function $\ell_C(\theta; z)$ described by Lemma 5.1 of \citet{song2020evading}.

\begin{figure}[h]
\centering
\includegraphics[width=.93\columnwidth]{figures/wine_plot.png}
         \caption{Linear regression on UCI wine quality dataset.}
\end{figure}
\label{fig:adult}

% Consider the transformation $f(\langle x, \theta \rangle; y) := \ell(\theta; z)$. When $f(\langle x, \theta \rangle; y) = \frac{1}{2}(y - x^T \theta)^2$ is the linear loss function,
% \begin{align*}
% f_C(\langle x, \theta \rangle; y)= \begin{cases} 
% - \frac{B}{||x||_2}\big[ \langle x, \theta \rangle - (y -  \frac{B}{||x||_2})\big] + f\big(y - \frac{B}{||x||_2}\big), \text{ for } \langle x, \theta \rangle \in (-\infty, y - \frac{B}{||x||_2}) \\
% f(\langle x, \theta \rangle), \text{ for } \langle x, \theta \rangle \in (y - \frac{B}{||x||_2}, y + \frac{B}{||x||_2}) \cap \mathbb{R} \\
%  \frac{B}{||x||_2}\big[ \langle x, \theta \rangle - (y +  \frac{B}{||x||_2})\big] + f\big(y + \frac{B}{||x||_2}\big), \text{ for } \langle x, \theta \rangle \in (y + \frac{B}{||x||_2}, \infty)
% \end{cases}
% \end{align*}

% where $f\big(y - \frac{B}{||x||_2}\big) = \frac{1}{2}\left(\frac{B}{||x||_2}\right)^2$

% and 

% $f\big(y + \frac{B}{||x||_2}\big) = \frac{1}{2}\left(-\frac{B}{||x||_2}\right)^2 = \frac{1}{2}\left(\frac{B}{||x||_2}\right)^2$

% write down clipped-gradient loss function for logistic and linear regression

% experimental set-up
% name hyperparameters for each alg
% LBFGS optimizer
% data pre-processing
% none for wine, normalize by row for adult (still private)

% \subsection{A Quick Primer on Differentially Private Hyperparameter Tuning}



